Object Referring in Visual Scene with Spoken Language

Object referring has important applications, especially for human-machine interaction. While having received great attention, the task is mainly attacked with written language (text) as input rather than spoken language (speech), which is more natural. This paper investigates Object Referring with Spoken Language (ORSpoken) by presenting two datasets and one novel approach. Objects are annotated with their locations in images, text descriptions and speech descriptions. This makes the datasets ideal for multi-modality learning. The approach is developed by carefully taking down ORSpoken problem into three sub-problems and introducing task-specific vision-language interactions at the corresponding levels. Experiments show that our method outperforms competing methods consistently and significantly. The approach is also evaluated in the presence of audio noise, showing the efficacy of the proposed vision-language interaction methods in counteracting background noise.

==> approach.tex <==

\section{Approach}
Our entire pipeline of the work is shown in Fig.~\ref{fig:pipeline}. Given an image and a human generated speech for referring objects, the goal of our work is to localize the corresponding object in the image. We approach the problem broadly in two ways: 1) Pipelined Approach as in Fig.~\ref{fig:pipeline}, 2) End-to-end SOR learning directly from speech (Sec.~\ref{subsection:end2endsor}). Pipelined approached can be viewed as two steps: a) Visually grounded speech recognition (Sec.~\ref{subsection:vgsr}) for transcribing speech to text b) Language based Object detection (Sec.~\ref{subsection:lod}) for localizing the object in the image, which we explain below.

\begin{figure}[tb!]
\centering
\adjustbox{trim={.09\width} {.25\height} {0.05\width} {.18\height},clip}{
\includegraphics[width=1.2\textwidth]{sbor_pipeline.pdf}}
\caption{The illustration of our complete pipelined approach for Speech based Object Referring. Given an image and speech data, VGSR performs speech recognition to output a text expression, conditioned on the visual input. LOD performs the object detection using the generated text.}
\label{fig:pipeline}
\end{figure} 


\subsection{Pipelined Speech-based Object Referring}
\label{subsection:pipelined}
\subsubsection{Visually grounded Speech Recognition}
\label{subsection:vgsr}

%\dengxincomment{a formulation probably? we formulate this as a ranking problem, similar to ~\cite{image:description:ranking}} 
There is a large body of work on visually grounded speech understanding or language understanding~\cite{Natural:Language:Commands,symbol:grounding:11}. In order to better show insights, we keep the method simple in this work by adopting a holistic ranking approach~\cite{image:description:ranking}. In particular, given an image and a speech data referring an object, we generate a list of alternatives for transcribed text and then use a simple ranking model to rank the alternatives based on the visual input. 

We use Google Cloud Speech API service~\footnote{\url{https://cloud.google.com/speech/}} for transcribing speech to text. For a given speech input, the tool yields a diverse set of transcribed text results obtained by diverse beam search as in Fig.~\ref{fig:pipeline}. Here, speech recognition results are proposed agnostic to the visual context. Nevertheless, we have a prior information that speech refers to an object in the image. Hence, we learn a similarity model to rank the speech recognition results conditioned on the image. The model is learned to score the set of transcribed alternatives using a regression loss. The inputs of the model are the embedded representations of image and text. The image features are extracted using CNN of VGG~\cite{vgg16} network while we use a two-layer LSTM with 300 hidden layer nodes each for textual features. Subsequently, image and textual features are subjected to element wise multiplication and a fully connected layer before the final layer which is a single node regression layer. This layer outputs the score for the speech recognition alternatives.
For training, we use the google speech recognition alternatives of GoogleRef train set, generated in the same way from Google API. For each expression in train set, we calculate a score for all the alternatives using the metrics: BLEU~\cite{papineni2002bleu}, ROUGE~\cite{lin2004rouge}, METEOR~\cite{banerjee2005meteor} and CIDEr~\cite{vedantam2015cider}, which are the well-known evaluation metrics in NLP domain. In Fig.~\ref{fig:metrics_hist}, we plot the histogram of the scores of the metrics having mapped to the range of $[0,1]$. The google speech alternatives have little differences with the ground truth expressions. We experiment to determine which metric captures these subtle differences. In Fig.~\ref{fig:metrics_hist}, the lesser the skewness in the score distribution, the better the metric is sensitive to the subtle differences. CIDEr seems to have a low skew. Consequently, we use CIDEr scores for training the model because they have equi-distribution over the entire range of scores compared to other three as shown in Fig.~\ref{fig:metrics_hist}. In the inference stage, for a given image and the set of alternatives, we use the output regression scores to rank the alternatives. Thus, we have  Visually Grounded Speech Recognition where we conduct the speech recognition with the context of image.

\begin{figure}[tb!]
     \begin{center}
     \begin{tabular}{cccc}
     \hspace{-1mm}
     \raisebox{-\totalheight}{\includegraphics[width=0.23\textwidth, height=20mm, trim={10mm 0mm 10mm 10mm},clip]{distribution_bleu_10.png}}
      &  \hspace{-2mm}
      \raisebox{-\totalheight}{\includegraphics[width=0.23\textwidth, height=20mm, trim={10mm 0mm 10mm 10mm},clip]{distribution_rouge_10.png}}
      & 
\hspace{-2mm}
       \raisebox{-\totalheight}{\includegraphics[width=0.23\textwidth, height=20mm, trim={10mm 0mm 10mm 10mm},clip]{distribution_meteor_10.png}}
        & \hspace{-2mm}
       \raisebox{-\totalheight}{\includegraphics[width=0.23\textwidth, height=20mm, trim={0mm 0mm 10mm 10mm},clip]{distribution_cider_10.png}} \\
      % \\
      	 \vspace{-2mm}
      \hspace{-1mm}    \small{BLEU noise 10\%} &  \hspace{-2mm}\small{ROUGE noise 10\%} &  \hspace{-2mm} \small{METEOR noise 10\%} &  \hspace{-1mm} \small{CIDEr noise 10\%}\\ 
      \end{tabular}
      \caption{Distributions of scores evaluated by comparing  the text alternatives by ASR for the recorded speeches (with 10\% added noise) to ground-truth expressions.}
\label{fig:metrics_hist}
\end{center}
\end{figure}

\subsubsection{Language based Object Detection}
\label{subsection:lod}
Given an image, referring expression and a set of bounding box object proposals in the image, our aim of Language based Object Detection(LOD) is to identify the bounding box location of the object that matches with the given expression. 
%Our aim in this part is to train a model to predict the bounding box location of the object in the image given the referring expression. 
The object detection, in general, has two main parts- generating object proposals and then selecting the ones based on the suitability to be an object. Following this notion, we use faster RCNN (FRCNN) object detector to propose the candidates. These candidates are later ranked by a complex model based on the given referring expression. We approach this task of LOD by a generative model.
%We use the global visual context, local object content and spatial information of the object as the feature from image  

\textbf{Generative approach} Following the work of Hu \textit{et al}~\cite{hu2016natural}, we perform the LOD task using a generative approach. Here, the model learns a scoring function that takes candidate regions, their spatial configurations and global context along with the given referring expression as input and then outputs scores for all candidate regions. The model chooses that candidate which maximizes the generative probability of the expression for the target object. The model architecture is same as that of \cite{hu2016natural}. We extract \textit{fc7} features of VGG-16~\cite{vgg16} net from bounding box location for object features and from whole image for global contextual feature. Textual features are extracted using a embedding layer which is also learned in an end-to-end fashion.

\subsection{End-to-end Speech-based Object Referring}
\label{subsection:end2endsor}
\textbf{Discriminative approach}
Inspired from the work on representation learning of speech data directly from speech such as~\cite{soundnet,speech:caption,speechVQA}, we design a discriminative model that tries to learn directly from raw speech and image data to perform SOR task. We extract the same set of features as in the case of generative approach. We concatenate the object features, spatial configurations and global contextual features into a single representation and passes through a fully connected layer to yield a fixed length vector representation for the visual part. For the speech part, we pass the raw speech signal through a series of 1D Convolutional Neural networks and a LSTM layer that outputs the vector representation for speech part. We tried different combination of networks such as similarity network~\cite{speech:caption}, MCB~\cite{multimodal:pooling}, etc. We have produced the results for MCB in Tab.~\ref{tab:result:SOR} which shows that this performs inferior compared to the pipelined SOR. Let us see the experiments in the next section.
%This vector is kept as the initial state for the input cells of two-layer LSTM. The LSTM takes word2vec~\cite{glove} vector representation of words of the expression and outputs softmax probabilities for the candidate region being a \textit{relevant} or a \textit{non-relevant} object.




==> dataset.tex <==

%--------------------------------------------------
\begin{table*}
\resizebox{2.0\columnwidth}{!}{
\centering
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multicolumn{2}{c}{Dataset}  & \#Images & \#Objects &Synthetic Speech & Real Speech & On-site Noise \\ \midrule
\multirow{2}{*}{GoogleRef}  & Train & $24698$ & $85474$  &\cmark &  \xmark & \xmark\\
 & Test &$4650$ & $9536$ & \cmark & \cmark & \xmark \\
\multirow{2}{*}{DrivingRef} & Train &$125$ & $500$ & \cmark & \cmark & \cmark \\
 & Test &$125$ & $500$  & \cmark & \cmark & \cmark \\
\bottomrule
\end{tabular}
}
\caption{Statistics of the two datasets.}
\label{tab:dataset-stats}
\end{table*}
%---------------------------------------------------------

Creating large datasets for Object Referring with Spoken Language (ORSpoken) is very labor intensive, given the fact that one need to annotate object location, issue language description and record speech description. A few choices are made in this work to scale the data collection: 1) Following previous work for language-based OR~\cite{mao2016generation,hu2016natural}, we use a simple bounding box to indicate the location of object; and 2) Following the success of synthetic data in many other vision tasks\cite{flow:chair,synthetic:text}, we construct hybrid speech recordings which contain sounding-realistic synthetic speeches for training and real human speeches for evaluation. Two datasets are used in this work, one focusing on scenarios for assistive robots and the other for automated cars. 

\subsection{GoogleRef}
\label{subsec:gref}

\textbf{Object Annotation}. As the first testbed, we choose to enrich the standard object referring dataset GoogleRef~\cite{mao2016generation} with speeches. GoogleRef contains $24,698$ images with $85,474$ associated referring expressions in the training set and $4,650$ images with $9,536$ associated referring expressions in the testing set. 

\textbf{Synthetic Speech}. Amazon Polly~\footnote{The voice of Joanna is used: \url{https://aws.amazon.com/polly/}} is used to generate the corresponding speech files for all referring descriptions. This TTS system produces high-quality realistic-sounding speech. It is nevertheless still simpler than real human speech due to the lack of tempo variation and ambient noise. We have thus recorded the real speeches for the testing set of GoogleRef. All speech files are in wav format, at 16 kHz.




\begin{figure}
     \begin{center}
     \begin{tabular}{cccc}
      \hspace{-1mm}
     \raisebox{-\totalheight}{\includegraphics[width=0.15\textwidth, height=20mm, trim={30mm 20mm 20mm 40mm},clip]{images/stop_here_001.png}}
      &  \hspace{-2mm}
      \raisebox{-\totalheight}{\includegraphics[width=0.15\textwidth, height=20mm, trim={30mm 20mm 20mm 40mm},clip]{images/stop_here_01.png}}
      & \hspace{-2mm}
       \raisebox{-\totalheight}{\includegraphics[width=0.15\textwidth, height=20mm, trim={30mm 20mm 20mm 50mm},clip]{images/stop_here_03.png}} \\
%         &  \hspace{-2mm}
%        \raisebox{-\totalheight}{\includegraphics[width=0.22\textwidth, height=20mm, trim={30mm 20mm 20mm 55mm},clip]{images/stop_here_05.png}} \\
           \hspace{-1mm}  (a)  original  &  \hspace{-2mm} (b) + 10\% noise &  \hspace{-2mm} (c) + 30\% noise \\  %\hspace{-2mm} (d) + 50\% noise\\ 
      \end{tabular}
      \caption{Audio waveforms of `stop here', with different levels of noise. }
      \label{fig:noisy:speech}
      \end{center}
      \end{figure}



\textbf{Real Speech}. We recorded real speech for all the referring expressions of GoogleRef by crowd-sourcing via Amazon Mechanical Turk(AMT). In AMT web interface, we show five text expressions for each Human Intelligence Task(HIT) and workers are instructed to speak out the expression and record each of the expression separately before submitting the HIT. Workers are asked to speak out as they are talking to a robot. We perform automatic validation by checking the length and volume of the recorded speeches to reject erroneous recordings due to inappropriate use of microphones. After each recording, we display the waveform of the recorded speech and an audio playback tool to hear back the recordings. We also keep a threshold for the amplitude of the audio signal to ensure the recording to attain certain volume level. Our automatic filter only accept the HIT only when all the five recordings are sufficiently long and the amplitude reaches the threshold. To further improve the quality of recordings, we also ran an initial round of recordings to qualify workers; only the qualified workers are allowed to our final recordings. 

%  To get a diverse set of recordings, we allowed the participation of workers from all countries and not restricting to English-speaking. 

\textbf{Noisy Speech}. To further study the performance of the method, we add different levels of noise to the speech files. The noise we mixed with the original speech files is selected randomly from the Urban8K dataset~\cite{urban8k}. This dataset contains 10 categories of ambient noise: air conditioner, car horn, children playing, dog bark, drilling, enging idling, gun shot, jackhammer, siren, and street music. For each original audio file, a random noise file is selected, and combined to produce a noisy audio expression:
\begin{equation}
  E_{noisy} = (1-\beta)*E_{original}  + \beta*Noise
  \label{equ:noise}
\end{equation}
where $\beta$ is the noise level. The noise audio files are sub-sampled to 16 kHz in order to match that of the speech audio file.  Both files are normalized before being combined so that contributions are strictly proportional to the noise level chosen. We study 3 noise levels: 0\%, 10\%, and 30\%.  A visualization of different noise levels can be seen in Fig. \ref{fig:noisy:speech}. 


\begin{figure}
\centering
\begin{tabular}{cccccc}
\hspace{-1.5mm}
\begin{adjustbox}{valign=t}
  \includegraphics[width=1.0in,height=0.9in]{driving_route.png}
\end{adjustbox}
&
\hspace{-3mm}
\begin{adjustbox}{valign=t}
\begin{tabular}{@{}c@{}}
  \includegraphics[width=1.0in,height=0.6in]{highway.jpg}\\[2ex]
  \includegraphics[width=1.0in,height=0.2in, trim={30mm 20mm 20mm 30mm},clip]{./images/noise_highway.png}
\end{tabular}
\end{adjustbox}
&
\hspace{-3mm}
\begin{adjustbox}{valign=t}
\begin{tabular}{@{}c@{}}
  \includegraphics[width=1.0in,height=0.6in]{tunnel.jpg}\\[2ex]
  \includegraphics[width=1.0in,height=0.2in, trim={30mm 20mm 20mm 30mm},clip]{./images/noise_tunnel.png}
\end{tabular}
\end{adjustbox}
% &
% \hspace{-3mm}
% \begin{adjustbox}{valign=t}
% \begin{tabular}{@{}c@{}}
%   \includegraphics[width=1.2in,height=0.8in]{./images/tram.jpg}\\[2ex]
%   \includegraphics[width=1.2in,height=0.2in, trim={30mm 20mm 20mm 30mm},clip]{./images/noise_busycity.png}
% \end{tabular}
% \end{adjustbox}
\\
\text{(a) driving route}  & \text{(b) highway} & \text{(c) tunnel} \\ %& \text{(d) busy city} 
\end{tabular}
\caption{The driving route of our driving dataset, along with two exemplar visual scenes and the corresponding in-vehicle noise characteristics.}
\label{fig:driving:route}
\end{figure}

\subsection{DrivingRef Dataset} 
\label{subsec:drivingdataset}
\textbf{Object Annotation.} In order to have more realistic noise and to evaluate our method in human-vehicle communication, we have created a new dataset DrivingRef for driving scenario. We drove over a 90-minutes route covering highway, residential area, busy city and tunnels. Driving scenes were recorded by a camera mounted on the windshield of the car and the in-vehicle noise was recorded by a microphone mounting on the dashboard of the car.  Fig.~\ref{fig:driving:route} shows the driving route, along with samples of the visual scenes and the corresponding in-vehicle noises. We sampled the frames uniformly from the entire length of the recorded video. For annotation, we crowd-sourced to AMT to annotate bounding boxes for the objects on the sampled frames. In the AMT interface, we show the frame and workers are asked to draw tight bounding boxes around the object they would like to refer to. For each bounding box annotated, workers are asked to type a truthful, informative, relevant, and brief expression so that co-observers can find the referred objects easily and unambiguously. For each image, we ask them to annotate four objects along with their referring expressions. In total, we have annotated 1000 objects in 250 diverse images chosen out of the 10,000 recorded images.

\textbf{Synthetic \& Real Speech.} We recorded the text descriptions the same way as described in previous section for GoogleRef.

\textbf{Noisy Speech} In-vehicle noise characteristics are ascribed to many factors such as driving environment (i.e. highway, tunnel), driving states (i.e. speed, acceleration), and in-vehicle noise (i.e. background music). During the course of data collection for DrivingRef, we also recored the in-vehicle noise from inside the vehicle. We added this recorded real in-vehicle noise to the speeches according to Eq.~\ref{equ:noise}. Timestamps of images and the recorded noise audio are used to obtain the in-place noise clips for the corresponding images (visual scenes). 

In total, we have qualified 23 workers for the recording task. The statistics of the two datasets can be found in Table~\ref{tab:dataset-stats}. 

%The dataset is annotated with the guidance of  Gricean Maxims~\cite{Logic:conversation} for cooperative conversations between people. That is, the descriptions need to be truthful, informative, relevant, and brief for co-observers to find the target objects easily and unambiguously. ASR systems could be trained from naturally co-occurring visual context information,
      


==> tables_figures.tex <==

%\dengxincomment{a bar plot showing results of visually grounded selection vs. 1st, 2nd, 3rd, random ... alternative?}
%\dengxincomment{or a two-column table: left gt text, right the transcribed text, but we do these only when time allows}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[t]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{@{}llllllll@{}}
% \toprule
%  %&            & \multicolumn{2}{c}{HIT @ 1} &   &         \\ \cmidrule{3-4}
%  &Candidate Proposals& \multicolumn{1}{c}{5 } & \multicolumn{1}{c}{10 }& \multicolumn{1}{c}{30 }             \\ 
% % \cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(l){5-5}
% %&Method   & Acc@1    & Acc@1   & Acc@1 &  Acc@10  &  Acc@30   \\ 
% \midrule
% & Random & 14.609 & 10.087 & 6.091 \\
% \multicolumn{6}{l} {\textsc{Ground truth text}}  \\ 
% %& MCB\cite{multimodal:pooling} & 32.1& 31.24&28.34& 78.966 & - \\
% %& Sim model &  35.980& 33.87&33.035\\
% %& Sim model~\cite{karpathy2014deep}+FRCNN &  34.50& 34.38 -33.105&31.91 & 79.543 \\
% & NLOR\cite{hu2016natural} &  39.63& 38.28& 31.9  \\
% \midrule
% \multicolumn{6}{l} {\textsc{Transcribed Text: Polly}}  \\ 
% %& Sim model &  33.909& 33.548&30.719 \\
% %& Sim model+SRranking(Cider) &  33.738& 33.634&30.832 \\
% %& Sim model~\cite{karpathy2014deep}+FRCNN &34.376& 34.202& 31.77& 79.493 & - \\
% %& MCB\cite{multimodal:pooling} & 31.564 &30.146& 27.251& 78.966 & - \\
% & NLOR\cite{hu2016natural} &  37.207& 35.134& 28.812  \\
% & NLOR\cite{hu2016natural}+SRranking(Cider) &  37.995&36.524& 30.444 \\
% % \multicolumn{6}{l} {\textsc{Transcribed Text: Polly- Noise 5\%}}  \\ 
% % & Sim model &  33.637& 33.180&- & - &-\\
% % %& Sim model~\cite{karpathy2014deep}+FRCNN &-& 34.06& -& - & - \\
% % %& MCB\cite{multimodal:pooling} & - &-& -& - & - \\
% % & NLOR\cite{hu2016natural} &  36.573& 34.81& - & - \\

% \multicolumn{6}{l} {\textsc{Transcribed Text: Polly- Noise 10\%}}  \\ 
% %& Sim model~\cite{karpathy2014deep}+FRCNN &34.14& 33.98& -& 79.358 & - \\
% %& MCB\cite{multimodal:pooling} & - &-& -& - & - \\
% %& Sim model &  33.331& 33.048&30.268 \\
% %& Sim model +SRranking(Meteor)&  32.936& 32.573&29.732\\
% %& Sim model +SRranking(Rouge)&  33.089& 32.784&29.938\\
% %& Sim model +SRranking(Bleu)& 33.214& 32.839&30.097\\
% %& Sim model +SRranking&  33.307& 32.893&30.395 & - &-\\
% %& Sim model +SRranking(Cider)&  33.408& 33.083&30.367\\
% & NLOR\cite{hu2016natural} &  36.049& 33.866& 27.243 \\
% %& NLOR\cite{hu2016natural}+SRranking &  36.353& 34.542& 28.163 & - \\
% & NLOR\cite{hu2016natural}+SRranking(Cider) &  36.936& 34.962& 28.715  \\

% \multicolumn{6}{l} {\textsc{Transcribed Text: Polly- Noise 30\%}}  \\ 

% %& Sim model~\cite{karpathy2014deep}+FRCNN &33.44& 32.87& 30.428& 78.895 & - \\
% %& MCB\cite{multimodal:pooling}& - &-& -& - & - \\
% %& Sim model &  29.533& 28.918&26.731 \\
% %& Sim model +SRranking(Meteor)&  29.257& 28.506&-& - &-\\
% %& Sim model +SRranking(Rouge)&  30.013& 29.328&26.926& - &-\\
% %& Sim model +SRranking(Bleu)& 29.957& 29.333&26.887& - &-\\
% %& Sim model +SRranking(Cider)&  29.970& 29.335&26.944\\
% %& Sim model +SRranking&  29.958& 29.266&26.970& - &-\\
% & NLOR\cite{hu2016natural} &  31.30& 28.68& 22.710  \\
% %& NLOR\cite{hu2016natural}+SRranking & 31.664& 29.505&23.433 & - \\
% & NLOR\cite{hu2016natural}+SRranking(Cider) & 32.405& 29.865&23.979 \\
% % \multicolumn{6}{l} {\textsc{Transcribed Text: Polly- Noise 50\%}}  \\ 
% % & Sim model &  23.563& 22.523&19.983\\
% % %& Sim model~\cite{karpathy2014deep}+FRCNN &32.748& 31.733-31.604& 28.754& 78.501 & - \\
% % %& MCB\cite{multimodal:pooling} & - &-& -& - & - \\
% % & NLOR\cite{hu2016natural} & 23.665& 20.896& 16.010  \\
% \midrule
% \multicolumn{6}{l} {\textsc{Transcribed Text: Arun}}  \\ 
% %& Sim model &  33.923& 33.282&30.469 \\
% %& Sim model+SRranking(Cider) &  33.681& 33.255&30.823 \\
% & NLOR\cite{hu2016natural} &  30.925& 27.448& 21.277 \\
% & NLOR\cite{hu2016natural}+SRranking(Cider) &  32.296& 29.243& 22.973\\
% \multicolumn{6}{l} {\textsc{Transcribed Text: Arun - Noise 10\%}}  \\ 
% %& Sim model &  32.371&32.013&28.994 \\
% %& Sim model+SRranking(Cider) &  32.738& 32.375&29.814 \\
% & NLOR\cite{hu2016natural} &  29.360& 26.113&19.539 \\
% & NLOR\cite{hu2016natural}+SRranking(Cider)&31.150& 27.234& 20.678\\
% \multicolumn{6}{l} {\textsc{Transcribed Text: Arun - Noise 30\%}}  \\ 
% %& Sim model &  29.567& 29.262&27.105 \\
% %& Sim model+SRranking(Cider) &  29.265& 29.080&26.337 \\
% & NLOR\cite{hu2016natural} &  24.460&20.523& 14.846 \\
% & NLOR\cite{hu2016natural}+SRranking(Cider) & 24.814& 21.118& 16.373 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Acc@1 represents the accuracy of grounding of text referring expressions on objects with IoU=$0.5$. The different methods are evaluated on GoogleRef dataset.}
% \label{tab:googleref-text}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cline{2-10}
%& Synthetic- noise 50\% &0.299& 0.459 &3.496 &0.397 &0.392 &0.380 &0.366  & - \\

%\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Real}}}& \multirow{ 2}{*}{0\%}  & Google API 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\tabcolsep}{3pt}
\begin{table}[!htb]
     \caption{Accuracy (Acc@1) of object referring with IoU=0.5. }
     
\begin{minipage}{.45\linewidth}  %
      \centering
\begin{tabular}{@{}llllllllll@{}}
 \multicolumn{8}{c}{(a) GoogleRef} \vspace{1mm} \\ 
\toprule
 %&            & \multicolumn{2}{c}{HIT @ 1} &   &         \\ \cmidrule{3-4}
& &       &         & \multicolumn{3}{c}{\# of Object Proposals }\\ 
& & Noise & Methods & \multicolumn{1}{c}{5 } & \multicolumn{1}{c}{10 }& \multicolumn{1}{c}{30 }             \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(l){5-7}
%&Method   & Acc@1    & Acc@1   & Acc@1 &  Acc@10  &  Acc@30   \\ 
\cline{1-8}
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Text}}} &  & \multirow{ 2}{*}{Clean} & Random & 14.609 & 10.087 & 6.091  \\
%\multicolumn{6}{l} {\textsc{Ground truth text}}  \\ 
%& Sim model~\cite{karpathy2014deep} & 9.25& 8.87& 10.25 \\
%& MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62& - & 40.37 \\
& &  & NLOR\cite{hu2016natural}  & \textbf{39.63}& \textbf{38.28}& \textbf{31.9} \\
%& &  & MCB\cite{multimodal:pooling}  & 32.1& 31.24&28.34 \\
\cline{1-8}
%\multicolumn{6}{l} {\textsc{Transcribed Text: Arun}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.5& 8.25& 7.5 \\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.75& 8.25& 7.5\\
%& MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62& 23.75 & 40.37 \\
\parbox[t]{2mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{Speech}}}  & \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Synthetic}}}  & \multirow{3}{*}{0\%}  & SR+NLOR &   37.207& 35.134& 28.812  \\
& & & Ours (SOR)   &  \textbf{37.995} & \textbf{36.524}  &  \textbf{30.444}  \\
& & & Ours (End)   & 32.54 &31.73& 28.28\\

%& NLOR+SRranking &  -& -& - & -&- \\

\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Polly- Noise 5\%}}  \\ 
%& NLOR\cite{hu2016natural} &  7.875& 6.5& 5.0 &20.625&- \\
%& NLOR+SRranking &  -& -& - & -&- \\

%\multicolumn{6}{l} {\textsc{ Polly- Noise 10\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &9.25& 8.25& 7.0 \\
%& Sim model~\cite{karpathy2014deep}+SRranking &8.25& 8.25& 6.5 \\
& & \multirow{2}{*}{10\%} & SR+NLOR  &  36.049& 33.866& 27.243 \\
%& NLOR+SRranking &  6.875& 6.37& 4.37& 20.25&- \\
& & & Ours (SOR)   &  \textbf{36.353}&  \textbf{34.542}&  \textbf{28.163} \\
%& & & Ours (End)   & 32.548 &31.733& 28.285 \\
\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Polly- Noise 30\%}}  \\
%& Sim model~\cite{karpathy2014deep} &9.0& 8.25& 6.75 \\
%& Sim model~\cite{karpathy2014deep}+SRranking &8.25& 8.0& 6.75 \\
& & \multirow{2}{*}{30\%} & SR+NLOR &   31.30& 28.68& 22.710  \\
%& NLOR+SRranking &  6.0& 5.5& 3.75 & 19.125&- \\
& & & Ours (SOR)  &    \textbf{31.664}&  \textbf{29.505}& \textbf{23.433}  \\
%& & & Ours (End)  & 32.548 &31.733& 28.285 \\

\cline{2-8}
& \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Real}}}& \multirow{2}{*}{0\%}   & SR+NLOR &  30.925& 27.448& 21.277  \\
& & & Ours (SOR)  &  \textbf{32.296}&  \textbf{29.243}&  \textbf{22.973} \\

%\multicolumn{6}{l} {\textsc{ Arun- Noise 5\%}}  \\ 
%& NLOR\cite{hu2016natural} &  5.875&5.375& 3.125 & 16.25&- \\
%& NLOR+SRranking &  -& -& - & -&- \\
\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Arun- Noise 10\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.5& 8.5&7.25 \\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &9.0&8.75&7.75 \\
& & \multirow{2}{*}{10\%} & SR+NLOR  & 29.360& 26.113&19.539 \\
& & & Ours (SOR)  & \textbf{31.150}&  \textbf{27.234}&  \textbf{20.678} \\

\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Arun- Noise 30\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.75& 8.25&7.25 \\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.75& 8.5&7.5\\
& & \multirow{2}{*}{30\%}   & SR+NLOR &  24.460&20.523& 14.846  \\
& & & Ours (SOR)  &   \textbf{24.814}&  \textbf{21.118}&  \textbf{16.373}  \\

%\multicolumn{6}{l} {\textsc{ Arun- Noise 50\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &7.25& 6.0&5.0 \\
%& NLOR\cite{hu2016natural} &  5.75& 5.25& 3.5  \\
%\multicolumn{6}{l} {\textsc{Transcribed Text: Polly}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.5& 8.5& 6.5\\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.5& 8.25& 6.75\\
%& MCB\cite{multimodal:pooling} & - &8.75& 8.625& - & 40.37 \\

%\multicolumn{6}{l} {\textsc{ Polly- Noise 50\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &9.0& 8.0&6.5 \\
%& NLOR\cite{hu2016natural} &  10.75& 12.0& 10.75  \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
     % driving dataset 
 \begin{minipage}{.45\linewidth} %
      \centering
\begin{tabular}{@{}llllllllll@{}}
 \multicolumn{8}{c}{(b) DrivingRef} \vspace{1mm} \\ 
\toprule
 %&            & \multicolumn{2}{c}{HIT @ 1} &   &         \\ \cmidrule{3-4}
& &       &         & \multicolumn{3}{c}{\# of Object Proposals }\\ 
& & Noise & Methods & \multicolumn{1}{c}{5 } & \multicolumn{1}{c}{10 }& \multicolumn{1}{c}{30 }             \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(l){5-7}
%&Method   & Acc@1    & Acc@1   & Acc@1 &  Acc@10  &  Acc@30   \\ 
\cline{1-8}
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Text}}} &  & \multirow{ 2}{*}{Clean} & Random & 5.12 & 3.5 & 1.62 \\
%\multicolumn{6}{l} {\textsc{Ground truth text}}  \\ 
%& Sim model~\cite{karpathy2014deep} & 9.25& 8.87& 10.25 \\
%& MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62& - & 40.37 \\
& &  & NLOR\cite{hu2016natural} &  \textbf{13.75}& \textbf{16.5}& \textbf{14.75} \\
%& & & MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62 \\

\cline{1-8}
%\multicolumn{6}{l} {\textsc{Transcribed Text: Arun}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.5& 8.25& 7.5 \\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.75& 8.25& 7.5\\
%& MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62& 23.75 & 40.37 \\
\parbox[t]{2mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{Speech}}}  & \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Synthetic}}}  & \multirow{3}{*}{0\%}  & SR+NLOR &  13.75& 15.0& 12.75 \\
& & & Ours (SOR)   &  \textbf{14.25}& \textbf{16.25}& \textbf{14.25}  \\
& & & Ours (End) & 9.12 & 9.87 & 9.37\\

%& NLOR+SRranking &  -& -& - & -&- \\

\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Polly- Noise 5\%}}  \\ 
%& NLOR\cite{hu2016natural} &  7.875& 6.5& 5.0 &20.625&- \\
%& NLOR+SRranking &  -& -& - & -&- \\

%\multicolumn{6}{l} {\textsc{ Polly- Noise 10\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &9.25& 8.25& 7.0 \\
%& Sim model~\cite{karpathy2014deep}+SRranking &8.25& 8.25& 6.5 \\
& & \multirow{2}{*}{10\%} & SR+NLOR  &  13.5& 15.0& 13.0  \\
%& NLOR+SRranking &  6.875& 6.37& 4.37& 20.25&- \\
& & & Ours (SOR)   & \textbf{13.5}& \textbf{15.75}& \textbf{13.25} \\

\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Polly- Noise 30\%}}  \\
%& Sim model~\cite{karpathy2014deep} &9.0& 8.25& 6.75 \\
%& Sim model~\cite{karpathy2014deep}+SRranking &8.25& 8.0& 6.75 \\
& & \multirow{2}{*}{30\%} & SR+NLOR &  \textbf{14.25}& \textbf{14.5}& \textbf{11.75}  \\
%& NLOR+SRranking &  6.0& 5.5& 3.75 & 19.125&- \\
& & & Ours (SOR)  &  13.75& \textbf{14.5}& 11.5  \\

\cline{2-8}
& \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Real}}}& \multirow{2}{*}{0\%}   & SR+NLOR &  8.75& 9.0& 5.75  \\
& & & Ours (SOR)  & \textbf{11.5}& \textbf{12.75}& \textbf{10.5} \\
%\multicolumn{6}{l} {\textsc{ Arun- Noise 5\%}}  \\ 
%& NLOR\cite{hu2016natural} &  5.875&5.375& 3.125 & 16.25&- \\
%& NLOR+SRranking &  -& -& - & -&- \\
\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Arun- Noise 10\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.5& 8.5&7.25 \\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &9.0&8.75&7.75 \\
& & \multirow{2}{*}{10\%}   & SR+NLOR &  9.0& 9.5& 6.75  \\
& & & Ours (SOR)  &\textbf{11.5}& \textbf{13.25}& \textbf{8.5} \\
\cdashline{3-8}
%\multicolumn{6}{l} {\textsc{ Arun- Noise 30\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.75& 8.25&7.25 \\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.75& 8.5&7.5\\
& & \multirow{2}{*}{30\%}   & SR+NLOR &  6.5& 6.25&5.25  \\
& & & Ours (SOR)  &  \textbf{10.5}& \textbf{10.25}&\textbf{6.5}  \\
%\multicolumn{6}{l} {\textsc{ Arun- Noise 50\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &7.25& 6.0&5.0 \\
%& NLOR\cite{hu2016natural} &  5.75& 5.25& 3.5  \\
%\multicolumn{6}{l} {\textsc{Transcribed Text: Polly}}  \\ 
%& Sim model~\cite{karpathy2014deep} &8.5& 8.5& 6.5\\
%& Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.5& 8.25& 6.75\\
%& MCB\cite{multimodal:pooling} & - &8.75& 8.625& - & 40.37 \\

%\multicolumn{6}{l} {\textsc{ Polly- Noise 50\%}}  \\ 
%& Sim model~\cite{karpathy2014deep} &9.0& 8.0&6.5 \\
%& NLOR\cite{hu2016natural} &  10.75& 12.0& 10.75  \\
\bottomrule
\end{tabular}
\end{minipage}
\label{tab:result:SOR}
\end{table}


% \begin{table}[t]
% \centering
% \resizebox{0.7\columnwidth}{!}{

% \begin{tabular}{@{}lllllll@{}}
% \toprule
%  %&            & \multicolumn{2}{c}{HIT @ 1} &   &         \\ \cmidrule{3-4}
%  &Candidate Proposals& \multicolumn{1}{c}{5 } & \multicolumn{1}{c}{10 }& \multicolumn{1}{c}{30 }             \\ 
% % \cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(l){5-7}
% %&Method   & Acc@1    & Acc@1   & Acc@1 &  Acc@10  &  Acc@30   \\ 
% \midrule
% & Random & 5.12 & 3.5 & 1.62 \\
% \multicolumn{6}{l} {\textsc{Ground truth text}}  \\ 
% & Sim model~\cite{karpathy2014deep} & 9.25& 8.87& 10.25 \\
% %& MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62& - & 40.37 \\
% & NLOR\cite{hu2016natural} &  13.75& 16.5& 14.75 \\

% \midrule
% \multicolumn{6}{l} {\textsc{Transcribed Text: Arun}}  \\ 
% & Sim model~\cite{karpathy2014deep} &8.5& 8.25& 7.5 \\
% & Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.75& 8.25& 7.5\\
% %& MCB\cite{multimodal:pooling} & 9.12 &8.75& 8.62& 23.75 & 40.37 \\
% & NLOR\cite{hu2016natural} &  8.75& 9.0& 5.75  \\
% & NLOR+SRranking(Cider) & 11.5& 12.75& 10.5 \\
% %\multicolumn{6}{l} {\textsc{ Arun- Noise 5\%}}  \\ 
% %& NLOR\cite{hu2016natural} &  5.875&5.375& 3.125 & 16.25&- \\
% %& NLOR+SRranking &  -& -& - & -&- \\

% \multicolumn{6}{l} {\textsc{ Arun- Noise 10\%}}  \\ 
% & Sim model~\cite{karpathy2014deep} &8.5& 8.5&7.25 \\
% & Sim model~\cite{karpathy2014deep}+SRranking(Cider) &9.0&8.75&7.75 \\
% & NLOR\cite{hu2016natural} &  9.0& 9.5& 6.75  \\
% & NLOR+SRranking(Cider) &11.5& 13.25& 8.5 \\

% \multicolumn{6}{l} {\textsc{ Arun- Noise 30\%}}  \\ 
% & Sim model~\cite{karpathy2014deep} &8.75& 8.25&7.25 \\
% & Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.75& 8.5&7.5\\
% & NLOR\cite{hu2016natural} &  6.5& 6.25&5.25  \\
% & NLOR+SRranking(Cider) &  10.5& 10.25&6.5  \\

% %\multicolumn{6}{l} {\textsc{ Arun- Noise 50\%}}  \\ 
% %& Sim model~\cite{karpathy2014deep} &7.25& 6.0&5.0 \\
% %& NLOR\cite{hu2016natural} &  5.75& 5.25& 3.5  \\
% \midrule
% \multicolumn{6}{l} {\textsc{Transcribed Text: Polly}}  \\ 
% & Sim model~\cite{karpathy2014deep} &8.5& 8.5& 6.5\\
% & Sim model~\cite{karpathy2014deep}+SRranking(Cider) &8.5& 8.25& 6.75\\
% %& MCB\cite{multimodal:pooling} & - &8.75& 8.625& - & 40.37 \\
% & NLOR\cite{hu2016natural} &  13.75& 15.0& 12.75 \\
% & NLOR\cite{hu2016natural}+SRranking(Cider) &  14.25& 16.25& 14.25  \\
% %& NLOR+SRranking &  -& -& - & -&- \\

% %\multicolumn{6}{l} {\textsc{ Polly- Noise 5\%}}  \\ 
% %& NLOR\cite{hu2016natural} &  7.875& 6.5& 5.0 &20.625&- \\
% %& NLOR+SRranking &  -& -& - & -&- \\

% \multicolumn{6}{l} {\textsc{ Polly- Noise 10\%}}  \\ 
% & Sim model~\cite{karpathy2014deep} &9.25& 8.25& 7.0 \\
% & Sim model~\cite{karpathy2014deep}+SRranking &8.25& 8.25& 6.5 \\
% & NLOR\cite{hu2016natural} &  13.5& 15.0& 13.0  \\
% %& NLOR+SRranking &  6.875& 6.37& 4.37& 20.25&- \\
% & NLOR+SRranking(Cider) & 13.5& 15.75& 13.25 \\

% \multicolumn{6}{l} {\textsc{ Polly- Noise 30\%}}  \\
% & Sim model~\cite{karpathy2014deep} &9.0& 8.25& 6.75 \\
% & Sim model~\cite{karpathy2014deep}+SRranking &8.25& 8.0& 6.75 \\
% & NLOR\cite{hu2016natural} &  14.25& 14.5& 11.75  \\
% %& NLOR+SRranking &  6.0& 5.5& 3.75 & 19.125&- \\
% & NLOR+SRranking(Cider) &  13.75& 14.5& 11.5  \\

% %\multicolumn{6}{l} {\textsc{ Polly- Noise 50\%}}  \\ 
% %& Sim model~\cite{karpathy2014deep} &9.0& 8.0&6.5 \\
% %& NLOR\cite{hu2016natural} &  10.75& 12.0& 10.75  \\
% \bottomrule
% \end{tabular}
% }
% \caption{Acc@K represents the accuracy of grounding of text referring expressions on objects with IoU=$0.5$. The different methods are evaluated on TRACE dataset.}
% \label{tab:Ours-text}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb!]
     \begin{center}
     \begin{tabular}{cccc}
      \hspace{-1mm} 
     \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={30mm 40mm 60mm 20mm},clip]{demo_20_4.jpg}}
      & \hspace{-2mm}
      \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 30mm 50mm 20mm},clip]{demo_51_2.jpg}}& \hspace{-2mm}
       \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 50mm 60mm 20mm},clip]{demo_86_1.jpg}} & \hspace{-2mm}
        \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 20mm 20mm 20mm},clip]{demo_35_0.jpg}} \\ 
        \hspace{-1mm}    \tiny{laptop the bed man is using} &  \hspace{-2mm}\tiny{green t-shirt talking to two other men} &  \hspace{-2mm} \tiny{the silver vehicle next to a green truck} &  \hspace{-2mm} \tiny{keyboard on the laptop}\\ 

 \hspace{-1mm}
     \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={30mm 40mm 60mm 20mm},clip]{demo_115_2.jpg}}
      &     \hspace{-2mm}
      \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 30mm 50mm 20mm},clip]{demo_122_0.jpg}}
      &  \hspace{-2mm}
       \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 50mm 60mm 20mm},clip]{demo_144_2.jpg}}
         &  \hspace{-2mm}
        \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 20mm 20mm 20mm},clip]{demo_150_2.jpg}} \\ 
        \hspace{-1mm}    \tiny{red car moves ahead on} &  \hspace{-2mm}\tiny{silver car parked close to us} &  \hspace{-2mm} \tiny{blue signboard on the top left most} &  \hspace{-2mm} \tiny{lane}\\    
      \end{tabular}  \vspace{-2mm}
      \caption{Qualitative results on GoogleRef (top) and DrivingRef (bottom)) with real speech of the text descriptions shown. Red represents the predicted box and blue the ground-truth. }
\label{fig:qual_gref}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[tb!]
%      \begin{center}
%      \begin{tabular}{cccc}
      
%      \raisebox{-\totalheight}{\includegraphics[width=0.21\textwidth, height=20mm, trim={30mm 40mm 60mm 20mm},clip]{images/trace/demo_115_2.jpg}}
%       & 
%       \raisebox{-\totalheight}{\includegraphics[width=0.21\textwidth, height=20mm, trim={50mm 30mm 50mm 20mm},clip]{images/trace/demo_122_0.jpg}}
%       & 
%        \raisebox{-\totalheight}{\includegraphics[width=0.21\textwidth, height=20mm, trim={50mm 50mm 60mm 20mm},clip]{images/trace/demo_144_2.jpg}}
%          & 
%         \raisebox{-\totalheight}{\includegraphics[width=0.24\textwidth, height=20mm, trim={50mm 20mm 20mm 20mm},clip]{images/trace/demo_150_2.jpg}} \\ 
%         \hspace{-1mm}    \tiny{red car moves ahead on} &  \hspace{-0mm}\tiny{silver car parked close to us} &  \hspace{2mm} \tiny{blue signboard on the top left most} &  \hspace{-1mm} \tiny{lane}\\ 
%       \end{tabular}
%       \caption{Qualitative results of object localization using Real speech in DrivingRef dataset. Transcribed object referring expressions are provided below. Green and red boxes represent ground truth and predicted boxes. Right-most figure shows a failure case of speech recognition and LOD.}
% \label{fig:qual_trace}
% \end{center}
% \end{figure}


% audio results 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{@{}llllllll@{}}
% \toprule
%  %&            & \multicolumn{2}{c}{HIT @ 1} &   &         \\ \cmidrule{3-4}
%  &Candidate Proposals& \multicolumn{1}{c}{5 } & \multicolumn{1}{c}{10 }& \multicolumn{3}{c}{30 }             \\ 
%  \cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(l){5-7}
% &Method   & Acc@1    & Acc@1   & Acc@1 &  Acc@10  &  Acc@30   \\ \midrule
% & Random & 14.609 & 10.087 & 6.091& 39.34 & 68.29 \\
% %& Sim model~\cite{karpathy2014deep}+FRCNN & 32.179&31.276& 29.084& 79.023 & - \\%& 14.25 & 55.24   \\
% & Sim model~\cite{karpathy2014deep} & -&15.314& -&- & - \\
% & MCB\cite{multimodal:pooling} & 32.54 &31.73& 28.28& 78.43 & - \\
% \multicolumn{6}{l} {Noise-5\%}   \\ 
% %& Sim model~\cite{karpathy2014deep}+FRCNN & 32.179&31.265& 29.003& 79.019 & - \\
% & Sim model~\cite{karpathy2014deep} & -&-& -&- & - \\
% & MCB\cite{multimodal:pooling} & 32.54 &31.7337& 28.285& 78.435 & - \\
% \multicolumn{6}{l} {Noise-10\%}   \\ 
% %& Sim model~\cite{karpathy2014deep}+FRCNN & 32.179&31.265& 29.009& 79.009 & - \\
% & Sim model~\cite{karpathy2014deep} & -&13.922& -&- & - \\
% & MCB\cite{multimodal:pooling} & 32.548 &31.733& 28.285& 78.435 & - \\
% \multicolumn{6}{l} {Noise-30\%}   \\ 
% %& Sim model~\cite{karpathy2014deep}+FRCNN & 32.190&31.254& 29.009& 78.976 & - \\
% & Sim model~\cite{karpathy2014deep} & -&9.547& -&- & - \\
% & MCB\cite{multimodal:pooling} & 32.548 &31.733& 28.285& 78.435 & - \\
% \multicolumn{6}{l} {Noise-50\%}   \\ 
% %& Sim model~\cite{karpathy2014deep}+FRCNN & 32.20&31.271& 28.976& 78.976 & - \\
% & Sim model~\cite{karpathy2014deep} & -&6.241& -&- & - \\
% & MCB\cite{multimodal:pooling} & 32.548 &31.733& -& - & - \\
% \multicolumn{6}{l} {Noise-100\%}   \\ 
% & Sim model~\cite{karpathy2014deep} & 32.23&-& 28.971& 78.986& - \\%& 14.25 & 55.24   \\
% & MCB\cite{multimodal:pooling} &- &-& -& - & - \\
% \bottomrule
% \end{tabular}
% }
% \caption{Acc@K represents the accuracy of grounding of audio referring expressions on objects with IoU=$0.5$. The different methods are evaluated on GoogleRef.}
% \label{tab:googleref-audio}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{@{}llllllll@{}}
% \toprule
%  %&            & \multicolumn{2}{c}{HIT @ 1} &   &         \\ \cmidrule{3-4}
%  &Candidate Proposals& \multicolumn{1}{c}{5 } & \multicolumn{1}{c}{10 }& \multicolumn{3}{c}{30 }             \\ 
%  \cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(l){5-7}
% &Method   & Acc@1    & Acc@1   & Acc@1 &  Acc@10  &  Acc@30   \\ \midrule
% & Random & 5.12 & 3.5 & 1.62& - & - \\
% \multicolumn{6}{l} {\textsc{Arun}}  \\ 
% & Sim model~\cite{karpathy2014deep} & 9.62&10.0& 10.37& 24.12 & 40.37 \\
% & MCB\cite{multimodal:pooling} & 9.12 &9.87& 9.37& 23.25 & 40.37 \\
% \multicolumn{6}{l} {\textsc{Polly}}  \\ 
% & Sim model~\cite{karpathy2014deep} & 9.62&10.0& 10.37& 24.12 & - \\
% & MCB\cite{multimodal:pooling} & 9.12 &9.87& 9.37& 23.25 & 40.37 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Acc@K represents the accuracy of grounding of audio(Arun) referring expressions on objects with IoU=$0.5$. The different methods are evaluated on TRACE dataset.}
% \label{tab:Ours-audio}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

